Every Pixel Counts: Unsupervised Geometry Learning with Holistic 3D Motion Understanding

Learning to estimate 3D geometry in a single image by watching unlabeled videos via deep convolutional network has made significant process recently. Current state-of-the-art (SOTA) methods, are based on the learning framework of rigid structure-from-motion, where only 3D camera ego motion is modeled for geometry estimation.However, moving objects also exist in many videos, e.g. moving cars in a street scene. In this paper, we tackle such motion by additionally incorporating per-pixel 3D object motion into the learning framework, which provides holistic 3D scene flow understanding and helps single image geometry estimation. Specifically, given two consecutive frames from a video, we adopt a motion network to predict their relative 3D camera pose and a segmentation mask distinguishing moving objects and rigid background. An optical flow network is used to estimate dense 2D per-pixel correspondence. A single image depth network predicts depth maps for both images. The four types of information, i.e. 2D flow, camera pose, segment mask and depth maps, are integrated into a differentiable holistic 3D motion parser (HMP), where per-pixel 3D motion for rigid background and moving objects are recovered. We design various losses w.r.t. the two types of 3D motions for training the depth and motion networks, yielding further error reduction for estimated geometry. Finally, in order to solve the 3D motion confusion from monocular videos, we combine stereo images into joint training. Experiments on KITTI 2015 dataset show that our estimated geometry, 3D motion and moving object masks, not only are constrained to be consistent, but also significantly outperforms other SOTA algorithms, demonstrating the benefits of our approach.

==> preliminaries.tex <==
\vspace{-0.3\baselineskip}
\section{Preliminaries}
\vspace{-0.1\baselineskip}
\label{sec:preliminaries}
In order to make the paper self-contained, we first introduce the preliminaries for unsupervised depth and optical flow estimation proposed in \cite{zhou2017unsupervised,yang2018aaai,wang2017occlusion}. The core underlying idea is inverse warping from target view to source views with awareness of 3D geometry or optical flow. Regularization terms are further applied on estimated depth/flow, which we will elaborate in the following paragraphs. 
%Here, we make the denotation the same with~\cite{zhou2017unsupervised} for consistency.

\textbf{Unsupervised depth estimation framework.}
 % From the multiple view geometry, we know that for a target view image $I_t$ and a source view image $I_s$, given an estimated depth map $D_t$ for $I_t$ and an estimated transformation $T_{t\rightarrow s} \in \hua{S}\hua{E}(3)$ from $I_t$ to $I_s$, for any pixel $p_t$ in $I_t$, the corresponding pixel $p_s$ in $I_s$ can be found through perspective projection, \ie $p_s \sim \pi(p_t)$. Then, given such a matching relationship, a synthesized target view $\hat{I_s}$ can be generated from $I_s$ through bilinear interpolation. Finally, by comparing the photometric error between the original target view $I_t$ and the synthesized one $\hat{I_s}$. We can supervise the prediction of $D_t$ and $T_{t\rightarrow s}$.
% \vspace{-0.1\baselineskip}
% % Zhou \etal~\cite{zhou2017unsupervised} used a depth CNN and a pose CNN to predict $D_t$ and $T_{t\rightarrow s}$ respectively, and make this process differentiable with respect to the two by adopting the spatial transform operation~\cite{jaderberg2015spatial}. 
% Formally, given multiple source views $\hua{S}=\{I_s\}$ from a video sequences close to $I_t$, the photometric loss \wrt $I_t$ can be formulated as,
% {\small
%   % \setlength{\abovedisplayskip}{4pt}
%   % \setlength{\belowdisplayskip}{\abovedisplayskip}
%   % \setlength{\abovedisplayshortskip}{0pt}
%   % \setlength{\belowdisplayshortskip}{2pt}
% \begin{align}
% \label{eqn:photometric}
% & \scr{L}_{vs}(D, \hua{T})\! =\! \sum\nolimits_{s}\sum\nolimits_{p_t\in I_t}\!|I_t(p_t) - \hat{I_s}(p_t)|, ~\text{s.t.} \any p_t, D(p_t) > 0
% \end{align}
% }
% where $\hua{T}$ is the set of transformations between $I_t$ to each of the source views in $\hua{S}$.

% % As the projected coordinates $p_s$ value is continuous, the pixel value of $p_t$ in synthetic view $\hat{I}_s$ is determined by bilinear interpolation from neighboring 4 points. For the network that estimates both depth map and transformation matrix, the view synthesis difference serves as supervision for training:

% % View synthesis loss measures the photometric difference between one view (target image) and the synthesized images from other views (source images). Such reconstruction loss enables self-learning from frame sequences. 
% % With the differentiable bilinear sampling proposed in \cite{jaderberg2015spatial}, the synthesis from source view to target view can be incorporated into the network. 
% % Specifically, for target view image $I_t$, given predicted target view depth $D_t$ and predicted transformation from target view to source view $T_{t\rightarrow s}$, for any pixel $p_t$ in target image, the corresponding pixel in source image $I_s$ is: $p_s \sim T_{t\rightarrow s}D_t(p_t)p_t$. As the projected coordinates $p_s$ value is continuous, the pixel value of $p_t$ in synthetic view $\hat{I}_s$ is determined by bilinear interpolation from neighboring 4 points. For the network that estimates both depth map and transformation matrix, the view synthesis difference serves as supervision for training:
% % \begin{align}
% % L_{vs}=\sum_{p_t}|I_t(p_t)-\hat{I}_s(p_t)|
% % \end{align}
% \vspace{-0.1\baselineskip}
% \textbf{Regularization of depth.} Nevertheless, supervision based solely on view synthesis is ambiguous, due to one pixel can match to many candidates.
% Thus, extra regularization is required to learn reasonable depth prediction. 
% One common strategy proposed by previous works \cite{godard2016unsupervised,zhou2017unsupervised} is to encourage the estimated depth to be locally similar when no significant image gradient exists. 
% For instance, in \cite{godard2016unsupervised}, the regularization of depth $D_t$ is formulated as: 
% {\small
%   % \setlength{\abovedisplayskip}{4pt}
%   % \setlength{\belowdisplayskip}{\abovedisplayskip}
%   % \setlength{\abovedisplayshortskip}{0pt}
%   % \setlength{\belowdisplayshortskip}{2pt}
% \begin{align}
% \label{eqn:regular}
% \scr{L}_{s}(D_t, 2) &= \sum_{p_t}\sum_{d \in {x, y}}\|\nabla^{2}_dD_t(p_t)\|_1e^{-\alpha|\nabla_dI(p_t)|}
% \end{align}
% }
% where $\scr{L}_{s}(D, 2)$ is a spatial smoothness term that penalizes L1 norm of second-order gradients of depth along both $x$ and $y$ directions in 2D space. Here, the number $2$ represents the 2nd order. 

% \begin{align}
% L_s=\sum_{p_t}\sum_{d\in x,y}|\bigtriangledown_d^2 D_t(p_t)|
% \end{align}

\textbf{Unsupervised optical flow estimation.} 
% Yang \etal~\cite{yang2018aaai} claim that the smoothness in \equref{eqn:regular} is still a too weak constrain to generate a good scene structure, especially when visualized under normal representation, as shown in 
% \figref{fig:example}(b), the predicted normals from~\cite{zhou2017unsupervised} varies on the surface of the ground. In their work, they further introduce a normal map $N_t$ for $I_t$, and a depth-normal consistency energy between $D_t$ and $I_t$ is proposed,
% {\small
%   % \setlength{\abovedisplayskip}{4pt}
%   % \setlength{\belowdisplayskip}{\abovedisplayskip}
%   % \setlength{\abovedisplayshortskip}{0pt}
%   % \setlength{\belowdisplayshortskip}{2pt}
% \begin{align}
% \label{eq:orthognal}
% &\scr{C}_{p_t}(D_t, N_t) = \sum\nolimits_{p_j\in\hua{N}(p_t)}\omega_{jt}\|(\phi(p_j) - \phi(p_t))^T  N(p_t)||^2 \nonumber
% \end{align}
% }
% where $\scr{N}(p_t)$ is a set of 8-neighbors of $p_t$. $\phi(p)$ is the back projected 3D point from 2D coordinate $p$. $\phi(p_j) - \phi(p_t)$ is a difference vector in 3D, and $\omega_{jt}$ weights the equation.
% Based on such an energy, they developed a differentiable depth-to-normal layer to estimate $N_t$ given $D_t$, and a normal-to-depth layer to re-estimate $D_t$ given $N_t$. By applying losses in \equref{eqn:photometric} and \equref{eqn:regular}, plus a first-order normal smootheness loss $\scr{L}_s(N_t, 1)$, $N_t$ can be supervised and $D_t$ can be better regularized with at least 8-neighbors. As shown in~\figref{fig:example}(d), their strategy yields better predicted depths and normals especially along surface regions. The depth and normal consistency same as in \cite{yang2018aaai} is incorporated into LEGO.
% For more details, we refer to the original paper due to the space limitation.


% Depth and normal are two tightly correlated features to describe the 3D scene layout. Yang \etal \cite{} has proposed to model such consistency 
%by minimizing a set of quadratic equations. For each pixel $p_i$, the objection function to minimize is written as: $\scr{L}_{p_i}(D, N)=||[..., \phi(p_i)-\phi(p_j), ...]^T \cdot N(p_i)||^2$, where $\phi(p_x)$ is the 3D point projected from 2D point $p_x$, $\phi(p_i)-\phi(p_j)$ is the difference vector in 3D space. $N(p_i)$ is a $3 \times 1$ vector representing the normal direction at pixel $p_i$, with $||N(p_x)||^2 = 1$. $p_j \in \scr{N}(p_i)$, $\scr{N}(p_i)$ is a set of neighboring points of $p_i$.
% with two inference layers: depth-to-normal, normal-to-depth layers. Mean cross product is implemented to infer normal from depth map. The normal at point $p_i$ is infered from neighboring points set $\scr{N}(p_i)$ as: 
% \begin{align}
% N(p_i) \sim \sum_{p_{jx} \in \scr{N}(p_i)}((\phi(p_i)-\phi(p_{j1}))\times(\phi(p_i)-\phi(p_{j2}))  \nonumber \\
% with ||N(p_i)||^2 = 1, p_{j1}\cdot p_{j2}=0
% \end{align}
% where $\phi(p_x)$ is the 3D point projected from 2D point $p_x$, $\phi(p_i)-\phi(p_j)$ is the difference vector in 3D space. $N(p_i)$ is a $3 \times 1$ vector representing the normal direction at pixel $p_i$.

%As normal ground truth is not available, normal-to-depth is required to receive geometrical supervision from view synthesis. 
% For given normal map $N$, solution of recovering depth $D$ is not unique, the predicted depth $D_o$ output from the network is used as a reference depth to reconstruct a new depth map $D_n$. $D_n(p_j)=\psi(D_o(p_i), N(p_i))$, where $p_j\in \scr{N}(p_i)$.
